The Fearless Journey [Draft]

Existing minimal Object-Oriented models (OO), like Featherweight Java (FJ), are valuable for modelling programs and designing new programming languages and tools. However, their utility in developing real-world programs is limited. We introduce the 'Fearless Heart', a novel object calculus preserving FJ's minimal and extensible nature while being more suited for constructing complex, real-world applications. To illustrate the extensibility of the Fearless Heart, we extend it with Reference Capabilities (RC), creating R-Fearless. It supports mutability and other side effects while retaining the reasoning advantages of functional programming and gaining support for features that are well-known to be enabled by RC, like automatic parallelism, caching and invariants. R-Fearless is still minimal enough to allow further extensions. It is an ideal foundation for constructing both practical systems and formal models.

==> metarule-preamble.tex <==
% \newcommand{\T}{\ensuremath{{\mathit{T}}}}
% \newcommand{\Sentence}{\ensuremath{\mathit{Ts}}}
% \newcommand{\Paragraph}{\ensuremath{\mathit{P}}}
% \newcommand{\Ctx}{\mathcal{E}}
% \newcommand{\Rule}{\ensuremath{\mathit{R}}}
% \newcommand{\Rules}{\ensuremath{\mathit{Rs}}}
% \newcommand{\Point}{\,\texttt{\textbf{-}\!\!\textbf{-}\!\!\textbf>}\,}
% \newcommand{\Stop}{\mbox{\texttt{\textbf{.}}}}
% \newcommand{\OS}{\mbox{\texttt{\textbf{[}}}}
% \newcommand{\CS}{\mbox{\texttt{\textbf{]}}}}
% \newcommand{\OC}{\mbox{\texttt{\textbf{\{}}}}
% \newcommand{\CC}{\mbox{\texttt{\textbf{\}}}}}
\newcommand{\Remember}[2]{\OC#1\CC\OS#2\CS}
\newcommand{\GetRule}[3]{\ensuremath{\mathit{rule}(#1) = #2\Point#3}}

\newcommand{\SelectRule}{\ensuremath{\mathit{apply}}}
\newcommand{\Apply}{\ensuremath{\mathit{apply}}}
\newcommand{\Match}{\ensuremath{\mathit{match}}}

\newcommand{\Triple}[3]{\ensuremath{\langle#1,\,#2,\,#3\rangle}}
\newcommand{\Pair}[2]{\ensuremath{\langle#1,\,#2\rangle}}

\newenvironment{Define}[3]{
    \newcommand{\Line}[3]{##1 & = & ##2 & \quad \text{##3}\\}%
    \newcommand{\LineIf}[3]{##1 & \text{iff} & ##2 & \quad \text{##3}\\}%
    \newcommand{\With}[2]{\ensuremath{ &  &\hspace{-#1ex} ##1 &
\hspace{-#2ex} \text{##2}}\\}%

    \par\vspace{1.5ex}
    \noindent\par\ensuremath{\overline{\,\textbf{Define}\,}\quad #3}
    \par\begin{math}\quad\begin{array}{l c l l }
}{
    \end{array}\end{math}\par\vspace{1.5ex}\par
    \let\Line\undefined%
    \let\With\undefined%
}

\newcommand{\RuleName}[1]{\ensuremath{\textsc{(#1)}}}
\newcommand{\metarule}[4]{
\vspace{0.1cm}
\noindent\hspace{-1.4ex}\ensuremath{%
  \begin{array}{l@{\quad}c@{\quad}l}%
    \rotatebox[origin=c]{90}{\textsc{(#1)}}\!\!\!\! & %
    \frac{%
      \begin{array}{@{}c@{}}%
        #2 % Premises.
      \end{array}%
    }{%
      \begin{array}{@{}c@{}}%
        #3 % Consequence.
      \end{array}%
    } &%
    \small\begin{array}{@{}l@{}}%
       #4 % Side conditions.
    \end{array}%
  \end{array}%
}}

\newcommand{\metaruleCompact}[3]{\noindent\ensuremath{%
  \begin{array}{l@{\quad}c@{\quad}l}%
    \frac{%
      \begin{array}{@{}c@{}}%
        #1 % Premises.
      \end{array}%
    }{%
      \begin{array}{@{}c@{}}%
        #2 % Consequence.
      \end{array}%
    } &%
    \small\begin{array}{@{}l@{}}%
       #3 % Side conditions.
    \end{array}%
  \end{array}%
}}

==> preamble.tex <==
\RequirePackage[]{listings}
\RequirePackage[]{xspace}
\RequirePackage[]{hyperref}
\RequirePackage[]{wrapfig}
\RequirePackage[]{graphicx}

\definecolor{bluekeywords}{rgb}{0.13,0.13,1}
\definecolor{greencomments}{rgb}{0,0.5,0}
\definecolor{redstrings}{rgb}{0.9,0,0}

\lstdefinestyle{codeStyle}{
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    numberstyle=\footnotesize\ttfamily,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    commentstyle=\color{greencomments},
    % keywordstyle=\color{bluekeywords},
    % stringstyle=\color{redstrings},
    tabsize=2,
    breakindent=0pt,
    basicstyle=\ttfamily,
    xleftmargin=1em,
}
\lstset{style=codeStyle}
\lstset{
    morecomment=[l]{//},
    morekeywords={
        imm,
        iso,
        read,
        mut,
        lent,
        readOnly,
        mdf,
        recMdf,
        alias,
        package,
    },
    columns=flexible
}

%------ grammar environment----------
\newenvironment{Grammar}{$\begin{array}[t]{lcll}}{\end{array}$}
\newcommand\ProductionDef{%
  %\scalebox{0.8}[1]{${:}{:}$}\scalebox{0.5}[1]{$=$}%
  \Coloneqq\,
  }
\newcommand{\Production}[3]{%
%
\!\!#1%
%
&%
\!\!\!\ProductionDef\!\!%
&%
%
#2%
&%
%
\mbox{{\small{#3}}}%
}
\newcommand{\MoreProduction}[2]{%
&&%
#1 
&%
\mbox{{\small{#2}}}%
}
\newcommand{\Terminal}[1]{%
\ensuremath{%
\mbox{%
  %\color{blue}
  \textbf{\texttt{#1}}%
  }%
}%
}
\newcommand{\NonTerminal}[1]{\ensuremath{\mathit{#1}}\xspace}
\newcommand\QQ[1]{\ensuremath{\text{\lstinline{#1}}}}
\newcommand\Q\lstinline

\newcommand\e{\NonTerminal{e}}
\newcommand\es{\NonTerminal{\overline{e}}}
\newcommand\Xs{\NonTerminal{\overline{X}}}
\newcommand\X{\NonTerminal{X}}
\newcommand\x{\NonTerminal{x}}
\newcommand\xs{\NonTerminal{\overline{x}}}
\newcommand\Ts{\NonTerminal{\overline{T}}}
\newcommand\T{\NonTerminal{T}}
\newcommand\Ms{\NonTerminal{\overline{M}}}
\newcommand\m{\NonTerminal{m}}
\newcommand\M{\NonTerminal{M}}
\newcommand\D{\NonTerminal{D}}
\newcommand\Ds{\NonTerminal{\overline{D}}}
\renewcommand\L{\NonTerminal{L}}
\newcommand\Ls{\NonTerminal{\overline{L}}}
\newcommand\Topd{\NonTerminal{Top}}
\newcommand\Tops{\NonTerminal{\overline{Top}}}
\newcommand\DM{\NonTerminal{DM}}
\newcommand\DMs{\NonTerminal{\overline{DM}}}
\newcommand\mtype{\NonTerminal{mtype}}
\newcommand\R{\NonTerminal{R}}
\newcommand\NT[1]{\NonTerminal{#1}}

\newcommand\OS{\QQ{[}\xspace}
\newcommand\CS{\QQ{]}\xspace}
\newcommand\OR{\QQ{(}\xspace}
\newcommand\CR{\QQ{)}\xspace}
\newcommand\OC{\ensuremath{\text{\lstinline|\{|}\!\!}\xspace}
\newcommand\CC{\ensuremath{\text{\lstinline|\}|}}\xspace}
\newcommand\fstop{\QQ{.}\xspace}
\newcommand\com{\QQ{,}\xspace}
\newcommand\point{\,\,\QQ{->}\xspace}
\newcommand\col{\QQ{:}\xspace}

\newcommand\imm{\text{\Q@imm@}\xspace}
\newcommand\mut{\text{\Q@mut@}\xspace}
\renewcommand\read{\text{\Q@read@}\xspace}
\newcommand\iso{\text{\Q@iso@}\xspace}

\newcommand\sName{\ensuremath{\QQ{'}\!x}}

\newcommand\PromP[1]{#1[\Uparrow^{\text{\textbf{p}}}]}
\newcommand\PromR[1]{#1[\Uparrow^{\text{\textbf{r}}}]}
\newcommand\Prom[1]{#1[\Uparrow]}

\input{metarule-preamble}
